Exploring Image Representation with Decoupled Classical Visual Descriptors

Exploring and understanding efficient image representations is a long-standing challenge in computer vision. While deep learning has achieved remarkable progress across image understanding tasks, its internal representations are often opaque, making it difficult to interpret how visual information is processed. In contrast, classical visual descriptors (e.g. edge, colour, and intensity distribution) have long been fundamental to image analysis and remain intuitively understandable to humans. Motivated by this gap, we ask a central question: Can modern learning benefit from these classical cues? In this paper, we answer it with VisualSplit, a framework that explicitly decomposes images into decoupled classical descriptors, treating each as an independent but complementary component of visual knowledge. Through a reconstruction-driven pre-training scheme, VisualSplit learns to capture the essence of each visual descriptor while preserving their interpretability. By explicitly decomposing visual attributes, our method inherently facilitates effective attribute control in various advanced visual tasks, including image generation and editing, extending beyond conventional classification and segmentation, suggesting the effectiveness of this new learning approach for visual understanding. Project page: https://chenyuanqu.com/VisualSplit/.

==> Revision.tex <==
Authors made claims on interpretability which cannot be fully supported and 
on the use of the term disantanglement, which is not in line with a common usage. 

As the authors mention in the rebuttal “Disentangle in our paper refers to the disentanglement/decomposition of the visual input into visual descriptors, rather than disentangling the latent representation, as in classical definition. 



The main focus of this paper is to explore how well traditional visual descriptors can represent an image through a learning framework, without accessing the original image." They also suggest they will "re-word the potentially misleading term".



Overall, the reviewers and the ACs appreciated the potential of the work, including the idea of re-discovering classical features that can indeed be quite interpretable and "coherent" with human perception




==> figures/experiments/brightness_result.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth, keepaspectratio]{figures/experiments/CVPR Figure Brightness.pdf}
     \vspace{1mm}
    \caption{Comparison of brightness editing results using modified grey-level histograms as guidance input with Stable Diffusion 1.5 (v\_prediction) with our method. Each column represents a different exposure compensation, $\epsilon$, with values ranging from $-3$ to $3$, followed by an equalized version. The original images are displayed in the central column. Each image's corresponding grey-level histogram is shown in the top right corner of each image. }
    \label{fig:brightness generation}
\end{figure*}

==> figures/experiments/pretained.tex <==

\begin{figure*}
    \centering
    \begin{subfigure}[t]{0.23\textwidth}
        \includegraphics[width=\textwidth]{figures/picked_output/80_rgb.png}
        \caption{Source RGB Image (unseen by the model)}
        \label{fig:pretrained raw}
    \end{subfigure}
    ~ % 添加这个符号来使子图并排显示，而不是换行
    \begin{subfigure}[t]{0.23\textwidth}
        \includegraphics[width=\textwidth]{figures/picked_output/80_edge.png}
        \caption{Source Edge}
        \label{fig:pretrained edge}
    \end{subfigure}
    ~ % 同上，继续保持子图并排
    \begin{subfigure}[t]{0.23\textwidth}
        \includegraphics[width=\textwidth]{figures/picked_output/80_hist.png}
        \caption{Source Intensity Hist}
        \label{fig:pretrained gray}
    \end{subfigure}
    ~ % 继续保持子图并排
    \begin{subfigure}[t]{0.23\textwidth}
        \includegraphics[width=\textwidth]{figures/picked_output/80_segmented_rgb.png}
        \caption{Source Colour Segmentation}
        \label{fig:pretrained colour}
    \end{subfigure}
    \hfill

    
    \begin{subfigure}[t]{0.23\textwidth}
        \includegraphics[width=\textwidth]{figures/picked_output/80_output.png}
        \caption{Reconstructed RGB}
        \label{fig:pretrained construction raw}
    \end{subfigure}
    ~ % 添加这个符号来使子图并排显示，而不是换行
    \begin{subfigure}[t]{0.23\textwidth}
        \includegraphics[width=\textwidth]{figures/picked_output/80_output_edge.png}
        \caption{Reconstructed Edge}
        \label{fig:pretrained construction edge}
    \end{subfigure}
    ~ % 同上，继续保持子图并排
    \begin{subfigure}[t]{0.23\textwidth}
        \includegraphics[width=\textwidth]{figures/picked_output/80_output_hist.png}
        \caption{Reconstructed Intensity Hist}
        \label{fig:pretrained construction gray}
    \end{subfigure}
    ~ % 继续保持子图并排
    \begin{subfigure}[t]{0.23\textwidth}
        \includegraphics[width=\textwidth]{figures/picked_output/80_output_colour_segmentation.png}
        \caption{Reconstructed Colour Segmentation}
        \label{fig:pretrained construction colour}
    \end{subfigure}

    \caption{Qualitative illustration of the second-order feature input. Edge (b), Gray-level histogram (c), and Colour Segmentation(d) can be extracted and processed from raw image (a), which are served as network inputs.}
    \label{fig:pretrained task}
\end{figure*}

==> figures/experiments/training_logger.tex <==
\begin{figure*}[t!]
    \centering
    \begin{subfigure}[b]{0.3\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/experiments/pretrained_logger.png}
        \caption{Pre-training stage loss over steps.}
        \label{fig:training_logger_pretraining}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.3\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/experiments/finetuning_logger.png} 
        \caption{Fine-tuning. Classification accuracy on ImageNet over steps.}
        \label{fig:training_logger_finetuning}
    \end{subfigure}
        \hfill
        \begin{subfigure}[b]{0.3\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/experiments/linear_probing_logger.png}
        \caption{Linear probing. Classification accuracy on ImageNet over steps.}
        \label{fig:training_logger_linear_probing}
    \end{subfigure}
    \caption{Training loggers in Log-form. X-axis is shown as log-form a) The pre-training logger, b) The fine-tuning logger, c) The linear probing logger. }
    \label{fig:training_logger}
\end{figure*}


==> figures/introduction/overall_figure.tex <==
\begin{figure}[!t]
    \centering
    \includegraphics[width=\textwidth]{figures/introduction/overall figure.png}
    \caption{Overall figures}
    \label{fig:overall figures}
\end{figure}

==> figures/methods/disentangle_example.tex <==

\begin{figure}[t]
    \centering
    \begin{subfigure}[b]{0.23\textwidth}
        \includegraphics[width=\textwidth]{figures/methods/raw.png}
        \caption{Raw Image}
        \label{fig:rep raw}
    \end{subfigure}
    ~ % 添加这个符号来使子图并排显示，而不是换行
    \begin{subfigure}[b]{0.23\textwidth}
        \includegraphics[width=\textwidth]{figures/methods/edge.png}
        \caption{Edge}
        \label{fig:rep edge}
    \end{subfigure}
    ~ % 同上，继续保持子图并排
    \begin{subfigure}[b]{0.23\textwidth}
        \includegraphics[width=\textwidth]{figures/methods/gray_level.png}
        \caption{Gray-level Hist}
        \label{fig:rep gray}
    \end{subfigure}
    ~ % 继续保持子图并排
    \begin{subfigure}[b]{0.23\textwidth}
        \includegraphics[width=\textwidth]{figures/methods/colour.png}
        \caption{4-bit Colour}
        \label{fig:rep colour}
    \end{subfigure}

    \caption{Qualitative illustration of the second feature input. Edge (b), Grey-level intensity histogram (c), and 4-bit Colour (d) can be extracted and processed from raw image (a), which are served as network inputs. In the 4-bit color illustration, the L channel is uniformly adjusted to a value of 50 for visualization purposes.}
    \label{fig:illustration}
\end{figure}

==> rebuttal/tables/convergence.tex <==
% \begin{table}
% \centering
% \caption{Comparison of Different Decoder Depth for Classification}
% \begin{tabularx}{1\linewidth}{|c|>{\centering\arraybackslash}X|>{\centering\arraybackslash}X|}
% \hline
% \textbf{block} & \textbf{Linear Probing} & \textbf{Fine-tuning}
%                                   \\ \hline

% 1  & 60.2 & 82.9   \\ \hline
% 2 & 68.8 & 83.4  \\ \hline
%     4 & 72.5 & 83.4  \\ \hline
%         8 & \textbf{74.0} & \textbf{83.5} \\ \hline
%             12 & 73.6 & 83.4\\
%             \hline
% \end{tabularx}
% \label{rebuttaltab: decoder depth}
% \end{table}




% \begin{table}
% \centering
% \caption{Decoder Depth Impact on Classification. }
\vspace{-3mm}
\begin{center}
    

\resizebox{0.5\linewidth}{!}{
 \begin{tabular}{l|c|c|c|c}
% \begin{tabularx}{1\linewidth}{|c|>{\centering\arraybackslash}X|>{\centering\arraybackslash}X|>{\centering\arraybackslash}X|>{\centering\arraybackslash}X|>{\centering\arraybackslash}X|}
% \hline
\hline
% {Length} &  128 &  256 & 512 & 768 & 1024 \\ \hline

% {Linear Probing}  &61.5 & 68.9 &  73.5 &  74.0 & \textbf{74.6}  \\ 
% {Fine-tuning}  &75.1 & 80.1  &  83.3 & 83.5 & \textbf{83.6}
%  \\ \hline  \hline 
{Clusters} &  2 &  4 & 6 & 8 \\ \hline

{Accuracy (\%)}  &60.0&  67.1&  \textbf{74.0} &  73.4
 \\ \hline % \hline 

 
\end{tabular}}
\end{center}
% \label{rebuttaltab: decoder depth}
\vspace{-1mm}
% \end{table}


==> rebuttal/tables/decoder_layer.tex <==
% \begin{table}
% \centering
% \caption{Comparison of Different Decoder Depth for Classification}
% \begin{tabularx}{1\linewidth}{|c|>{\centering\arraybackslash}X|>{\centering\arraybackslash}X|}
% \hline
% \textbf{block} & \textbf{Linear Probing} & \textbf{Fine-tuning}
%                                   \\ \hline

% 1  & 60.2 & 82.9   \\ \hline
% 2 & 68.8 & 83.4  \\ \hline
%     4 & 72.5 & 83.4  \\ \hline
%         8 & \textbf{74.0} & \textbf{83.5} \\ \hline
%             12 & 73.6 & 83.4\\
%             \hline
% \end{tabularx}
% \label{rebuttaltab: decoder depth}
% \end{table}




% \begin{table}
% \centering
% \caption{Decoder Depth Impact on Classification. }

\vspace{-3mm}
\begin{center}
    

\resizebox{0.7\linewidth}{!}{
 \begin{tabular}{l|c|c|c|c|c|c}
% \begin{tabularx}{1\linewidth}{|c|>{\centering\arraybackslash}X|>{\centering\arraybackslash}X|>{\centering\arraybackslash}X|>{\centering\arraybackslash}X|>{\centering\arraybackslash}X|}
% \hline
\hline
% {Length} &  128 &  256 & 512 & 768 & 1024 \\ \hline

% {Linear Probing}  &61.5 & 68.9 &  73.5 &  74.0 & \textbf{74.6}  \\ 
% {Fine-tuning}  &75.1 & 80.1  &  83.3 & 83.5 & \textbf{83.6}
%  \\ \hline  \hline 
{Block} &  1 &  2 & 4 & 8 & 12 & 24 \\ \hline

{Linear Probing}  &60.2&  68.8&  72.5 &  \textbf{74.0} & 73.6 & 73.4\\ 
{Fine-tuning}  &82.9 & 83.4 &  83.4 & \textbf{83.5}& 83.4&83.4
 \\ \hline % \hline 

 
\end{tabular}}
\end{center}
% \label{rebuttaltab: decoder depth}
\vspace{-1mm}
% \end{table}


==> rebuttal/tables/latent_vector_length.tex <==






% \begin{table}
% \centering
% \caption{Latent Vector Length Impact on Classification.}
\vspace{-3mm}
\begin{center}
    

\resizebox{0.7\linewidth}{!}{
 \begin{tabular}{l|c|c|c|c|c}
% \begin{tabularx}{1\linewidth}{|c|>{\centering\arraybackslash}X|>{\centering\arraybackslash}X|>{\centering\arraybackslash}X|>{\centering\arraybackslash}X|>{\centering\arraybackslash}X|}
% \hline
\hline
{Length} &  128 &  256 & 512 & 768 & 1024 \\ \hline

{Linear Probing}  &61.5 & 68.9 &  73.5 &  74.0 & \textbf{74.6}  \\ 
{Fine-tuning}  &75.1 & 80.1  &  83.3 & 83.5 & \textbf{83.6}
 \\ \hline  %\hline 
\end{tabular}}
\end{center}
% \label{rebuttaltab: vector length}
\vspace{-1mm}
% \end{table}







==> tables/experiments/classification.tex <==
% \begin{table}[]
% \label{tab:classification}
% \caption{Task Generalization on Classification. Top-1 class accuracy (\%) reported.}
% \vspace{-0.15cm}
% \begin{tabularx}{\textwidth}{l|>{\centering\arraybackslash}X>{\centering\arraybackslash}X>{\centering\arraybackslash}X}
% \toprule
% \textbf{Method}             & \textbf{ImageNet} & \textbf{Places} & \textbf{PASCAL} \\ 
% \midrule
% Autoencoder~\cite{vincent2010stacked}       &      18.0       &    15.7          &   44.0     \\
% Colourization~\cite{zhang2016colorful}        &      32.5        & 32.0       &      68.0  \\
% Split-brain Autoencoder~\cite{zhang2017split}&      36.4           &   34.9     &    68.5    \\
% Swin2SR~\cite{conde2022swin2sr}        &        41.1     &     ongoing(19:00)        &    82.0    \\
% \midrule
% \NAME Gaussian init  $R_{full}$      &   0.0               &  0.0      &    0.1    \\
% \NAME  $R_{E}$        &      18.2       &   20.6   &      40.6         \\
% \NAME  $R_G$ &       0.0      &    0.0  &        0.2        \\
% \NAME $R_C$    &      12.5       &   13.5   &      33.1         \\
% \midrule
% \NAME $R_{full}$ &      36.4       &   36.0   &       69.5        \\


% \bottomrule

% \end{tabularx}

% \end{table}
% \usepackage{colortbl}

% 有考虑左边放不同VIT架构的图，不知道时间来不来得及
\begin{table}[t]
\centering
\label{tab:classification}
\caption{Task Generalization on Classification. Top-1 class accuracy (\%) reported.}
\vspace{-0.15cm}
\begin{tabularx}{0.8\textwidth}{l|>{\centering\arraybackslash}X>{\centering\arraybackslash}X}
\toprule
\textbf{Method}             & Finetuning & Linear Probing \\ 
\midrule
\rowcolor{gray!20} 
scratch, our impl.&    82.0       &          0.1 \\
Split-brain Auto~\cite{zhang2017split}
       &     82.3        &   36.4 \\
MAE  &     83.6        &   72.4  \\
PeCo&        84.5           &    51.7   \\

\NAME  &     83.5        &     74.0     \\


\bottomrule

\end{tabularx}

\end{table}

==> tables/experiments/image_captioning.tex <==
% \begin{table}[]
% \label{tab:imagecaptioning}
% \caption{Image Captioning Performance. BLEU score (\%) recorded.}
% \vspace{-0.15cm}
% \begin{tabularx}{\textwidth}{l|>{\centering\arraybackslash}X|>{\centering\arraybackslash}X|>{\centering\arraybackslash}X}
% \toprule
%  Method                   & COCO & Flickr & NoCaps \\ 
%                     \midrule
% Autoencoder~\cite{vincent2010stacked}        &       $17.23 \pm 4.22$       &  $20.46 \pm 5.26$    &    $15.99 \pm 3.99$    \\
% Colourization~\cite{zhang2016colorful}         &     $20.63 \pm 4.23$        &   $23.96 \pm 5.17$   &   $18.25 \pm 4.16$            \\
% Split-brain Auto~\cite{zhang2017split}         &   $20.87 \pm 4.01$          &   $24.40 \pm 5.06$   &   $18.76 \pm 3.92$            \\
% Swin2SR~\cite{conde2022swin2sr}        &      $22.83 \pm 3.86$       &   $25.16 \pm 4.88$   &     $19.54 \pm 3.82$      \\
% \midrule
% \NAME Gaussian init  $R_{full}$       &  $6.20 \pm 2.44$         &  $8.82 \pm 3.49$    &   $5.45 \pm 2.57$            \\
% \NAME  $R_{E}$        &       $19.71 \pm 4.13$      &  $23.56 \pm 5.31$    &         $18.70 \pm 4.08$      \\
% \NAME  $R_G$ &         $6.28 \pm 4.33$    &  $9.51 \pm 5.09$    &        $6.52 \pm 4.27$       \\
% \NAME $R_C$    &        $18.98 \pm 6.79$    &  $22.29 \pm 6.83$    &       $15.90 \pm 6.64$        \\
% \midrule
% \NAME $R_{full}$ &       $24.51 \pm 4.42$      &   $27.62 \pm 5.27$    &          $22.48 \pm 4.46$     \\
% \bottomrule
% \end{tabularx}
% \end{table}


\begin{table}[ht]
\centering
\caption{Transfer learning Performance}
\begin{subtable}{0.45\linewidth}
\caption{Transfer learning image classification performance on Places dataset.}
\label{tab:image classification transfer learning}
\begin{tabularx}{\textwidth}{l|>{\centering\arraybackslash}X}
\toprule
\textbf{Method}             & Accuracy (\%)\\ 
\midrule
\rowcolor{gray!20}scratch, our impl.~\cite{conde2022swin2sr}        &   79.9       \\
Split-brain Auto~\cite{zhang2017split}         &       81.4        \\
MAE       &   82.5   \\
PeCo   &     82.4    \\

\NAME  &      82.7     \\
\bottomrule
\end{tabularx}
\end{subtable}
\hfill
\begin{subtable}{0.45\linewidth}
\caption{Transfer learning semantic segmentation  performance on ADE20K dataset.}
\label{tab:semantic segmentation transfer learning}
\begin{tabularx}{\textwidth}{l|>{\centering\arraybackslash}X}
\toprule
\textbf{Method}             & mIoU\\ 
\midrule
\rowcolor{gray!20}scratch, our impl.~\cite{conde2022swin2sr}        &  47.7             \\
Split-brain Auto~\cite{zhang2017split}     &  44.4              \\
MAE       &    48.4       \\
 PeCo   &   48.7    \\

\NAME  &     49.7        \\
\bottomrule
\end{tabularx}
\end{subtable}

\end{table}

==> tables/experiments/pretrained.tex <==
\begin{table}[]
\label{tab:pretrained performance}
\caption{Pretrained Performance}
\vspace{-0.15cm}
\begin{tabularx}{\textwidth}{l|c}

\toprule
 Task                   & Metrics \\ 
                    \midrule
Edge        &      \\
Gray-level Historgram  &              \\
4 bit Colour         &              \\
Reconstruction       &         \\
\bottomrule
\end{tabularx}
\end{table}

==> tables/experiments/superresolution.tex <==
% \begin{table}[]
% \label{tab:superresolution}
% \caption{Super-resolution Performance. PSNR/ SSIM reported.}
% \vspace{-0.15cm}
% \begin{tabularx}{\textwidth}{l|>{\centering\arraybackslash}X|>
% {\centering\arraybackslash}X|>{\centering\arraybackslash}X}
% \toprule
%    Method                & ImageNet & COCO & Places \\ 
% \midrule
% \rowcolor{gray!20} Swin2SR~\cite{conde2022swin2sr}        &       32.57/ 0.9186      &   31.94/ 0.9130   &        32.44/ 0.9190       \\
% \midrule
% Autoencoder~\cite{vincent2010stacked}        &         29.90/ 0.8992     &  28.18/ 0.8891   &  28.33/ 0.8917      \\
% Colourization~\cite{zhang2016colorful}          &        29.82/ 0.8985     &   27.39/ 0.8623   &       27.72/ 0.8707        \\
% Split-brain Autoencoder~\cite{zhang2017split} &         29.92/  0.9035   &   27.97/ 0.8876   &     28.25/ 0.8931          \\

% \NAME Gaussian init  $R_{full}$        &        27.14/ 0.8399    &   22.88/ 0.5615   &        23.28/ 0.5889       \\
% \NAME  $R_E$        &          28.15/ 0.8634   &   25.69/ 0.8037   &        26.11/ 0.8077       \\
% \NAME  $R_G$ &          27.14/ 0.8447  &   24.17/ 0.7042   &        25.09/ 0.7583       \\
% \NAME $R_C$    &        28.21/ 0.8626     &    27.74/ 0.8626  &         28.14/ 0.8667      \\
% \midrule
% \NAME $R_{full}$ &         30.04/0.8994    &   29.68/ 0.8903   &        30.08/ 0.8994       \\
% % \midrule
% % \midrule
% % ViTMAE        &      $\times 4$&       &      &        \\
% % Colourization         &  $\times 4$&           &      &               \\
% % Swin2SR        &    $\times 4$&   24.07/ 0.7128      &      &               \\
% % \midrule
% % Gaussian init        &   $\times 4$&          &      &               \\
% % E        &        $\times 4$&     &      &               \\
% % G &        $\times 4$&     &      &               \\
% % C    &      $\times 4$&       &      &               \\
% % \midrule
% % Combine &       $\times 4$&  23.75/0.6944    &      &               \\
% \bottomrule
% \end{tabularx}
% \end{table}

\begin{table}[]
\caption{Super-resolution Performance. PSNR/ SSIM reported.}
\label{tab:superresolution}
\vspace{-0.15cm}
\begin{tabularx}{\textwidth}{l|>{\centering\arraybackslash}X|>
{\centering\arraybackslash}X|>{\centering\arraybackslash}X}
\toprule
   Method                & ImageNet & COCO & Places \\ 
\midrule
\rowcolor{gray!20} Swin2SR~\cite{conde2022swin2sr}        &       32.57/ 0.9186      &   31.94/ 0.9130   &        32.44/ 0.9190       \\
\midrule
Autoencoder~\cite{vincent2010stacked}        &         29.90/ 0.8992     &  \underline{28.18}/ \underline{0.8891}   &  \underline{28.33}/ 0.8917      \\
Colourization~\cite{zhang2016colorful}          &        29.82/ 0.8985     &   27.39/ 0.8623   &       27.72/ 0.8707        \\
Split-brain Autoencoder~\cite{zhang2017split} &         \underline{29.92}/ \textbf{0.9035}   &   27.97/ 0.8876   &     28.25/ \underline{0.8931}          \\
\midrule
\NAME Gaussian init  $R_{full}$        &        27.14/ 0.8399    &   22.88/ 0.5615   &        23.28/ 0.5889       \\
\NAME  $R_E$        &          28.15/ 0.8634   &   25.69/ 0.8037   &        26.11/ 0.8077       \\
\NAME  $R_G$ &          27.14/ 0.8447  &   24.17/ 0.7042   &        25.09/ 0.7583       \\
\NAME $R_C$    &        28.21/ 0.8626     &    27.74/ 0.8626  &         28.14/ 0.8667      \\
\midrule
\NAME $R_{full}$ &         \textbf{30.04}/\underline{0.8994}    &   \textbf{29.68}/ \textbf{0.8903}   &        \textbf{30.08}/ \textbf{0.8994}       \\
% \midrule
% \midrule
% ViTMAE        &      $\times 4$&       &      &        \\
% Colourization         &  $\times 4$&           &      &               \\
% Swin2SR        &    $\times 4$&   24.07/ 0.7128      &      &               \\
% \midrule
% Gaussian init        &   $\times 4$&          &      &               \\
% E        &        $\times 4$&     &      &               \\
% G &        $\times 4$&     &      &               \\
% C    &      $\times 4$&       &      &               \\
% \midrule
% Combine &       $\times 4$&  23.75/0.6944    &      &               \\
\bottomrule
\end{tabularx}
\end{table}
